Training Trajectories of Language Models Across Scales

Scaling up language models has led to unprecedented performance gains, but little is understood about how the training dynamics change as models get larger. How do language models of different sizes learn during pre-training? Why do larger language models demonstrate more desirable behaviors? In this paper, we analyze the intermediate training checkpoints of differently sized OPT models (Zhang et al.,2022)--from 125M to 175B parameters--on next-token prediction, sequence-level generation, and downstream tasks. We find that 1) at a given perplexity and independent of model sizes, a similar subset of training tokens see the most significant reduction in loss, with the rest stagnating or showing double-descent behavior; 2) early in training, all models learn to reduce the perplexity of grammatical sequences that contain hallucinations, with small models halting at this suboptimal distribution and larger ones eventually learning to assign these sequences lower probabilities; 3) perplexity is a strong predictor of in-context learning performance on 74 multiple-choice tasks from BIG-Bench, and this holds independent of the model size. Together, these results show that perplexity is more predictive of model behaviors than model size or training computation.

==> sections/pos_er.tex <==
Identify tokens the perplexity of which stagnates, increases and decreases. 


\begin{equation}
    \text{PPL}_t
\end{equation}


Auto-regressive models' training objective provides signals on how well the models have learned to predict the current token based on previous contexts. Normally we aggregate the predicted loss of all tokens to calculate the perplexity to represent the language model's ability~\citet{rae2021scaling}. Looking at perplexity in aggregate is informative, categorizing the tokens into a certain language phenomenon might provide a more complete and interpretable description of the learning trajectories of these models. In this section, we look into two specific language phenomena, part-of-speech tags and named entities, and partition the improvement of the log-likelihood on one validation dataset into different types of tokens. 

For a given corpus $\mathcal{T}$ that contains $n$ tokens, a checkpoint gives a log like-score score to each token $t$ based on the context of the token; the perplexity of all tokens is $\text{PPL}_{\mathcal{T}} = P(t_1 t_2 \cdots t_n)^{-\frac{1}{n}} = \exp(-\frac{1}{n}\sum_i^n nll_i)$ where $nll$ denotes the negative log-likelihood of a token. For a specific language phenomenon, we calculate its perplexity by only aggregating the tokens associated with this language phenomenon. For example, the perplexity of nouns is 
$$
\text{PPL}_{\text{Noun}} = \exp(-\frac{1}{\sum{\mathbbm{1}(t_i \text{is Noun})}}\sum_i^n \mathbbm{1}(t_i \text{is Noun}) \cdot nll_i).
$$ 

As the slope in the perplexity curve does not faithfully reflect the learning speed due to its exponentiality, we also evaluate the percentage of contribution each type of tag improves the perplexity in aggregate between two consecutive checkpoints. 

$$
\%_{\text{Noun}} = \frac{ll_{\text{Noun}}^{c_1} - ll_{\text{Noun}}^{c_2}}{ll^{c_1} - ll^{c_2}},
$$
where $ll_{\text{Noun}}^{c}$ is the log-likelihood of the corpus $\mathcal{T}$ with only nouns at checkpoint $c$, and $ll^{c}$ is the log-likelihood of the corpus $\mathcal{T}$ at checkpoint $c$.

Generally, training a large model to a level of perplexity requires more computation than small models, which coincides with the findings in \citet{hoffmann2022training}. For part-of-speech tags, We observe that adjectives have an exceptionally high perplexity, while verbs and nouns show a much lower perplexity. This is expected since entropy for adjectives is intrinsically higher than verbs and nouns. Digging deep into the verb category, VBG, denoting verbs with a gerund or present participle, has a very high perplexity. The percentage of log-likelihood improvement of NN and NNP almost adds up to one, indicating that almost all the computation flows to improve predictions for nouns. For the majority of the part-of-speech tags, the improvement percentage is rather insignificant. Named entities learn much faster than average at the final stage of training, though only make up of 10\% of the tokens, the contribution percentage reaches to up 60\%. 
We present the results across 6 OPT model sizes in \autoref{fig:pos-ner}. 

\noindent
{\color{red} \rule{\linewidth}{0.5mm}}
\colorbox{orange}{\textbf{TODO items:}}
\begin{itemize}
    \item \st{get results from step 4k to 40k, now we only have results from 40k to 140k}
    \item are named entities all nouns? \mz{named entities are proper nouns} % look more carefully into the graph and make sure the percentage is correct
    \item understand why JJ and VBG are hard to learn (entropy?, by checking the entropy of the distribution, these tokens might naturally have more uncertainty. or because there exists a token that has a much higher probability? basically it's worth examine the full distribution of the predicted token, which might give us hints on why at some point generation starts to get worse. ) % the same statistics we did previously, which token has the highest entropy? ing or the verb? 
    \item why are named entities hard to learn, is it because they are rare in training data? is it hard to identify it is this named entity or hard to memorize the entity. The diff between first appearance and after! The diff between first token and second/third tokens
    \item do different-sized models learn differently?
    \item list out the tokens/entities that lead to the highest perplexity
    \item draw the connection of nouns and computation, and make an argument that simply learning the nouns is not ideal!
\end{itemize}
\noindent

\colorbox{orange}{\textbf{Stretch goals:}}
\begin{itemize}
    \item How can we connect it to downstream task performance?
    \item Implications for generation? why at some point the model would more likely to shift away from the topic?
\end{itemize}

{\color{red} \rule{\linewidth}{0.5mm}}


\begin{figure}
    \begin{subfigure}{\linewidth}
    \includegraphics[width=.47\linewidth]{images/pos-ppl-flops.png} \hfill
    \includegraphics[width=.47\linewidth]{images/pos-cont.png}
    \caption{Part-of-speech tags. Left: slide 4; right: slide 26}
    \end{subfigure}\par\medskip
    \begin{subfigure}{\linewidth}
    \includegraphics[width=.47\linewidth]{images/ner-ppl-steps.png} \hfill
    \includegraphics[width=.47\linewidth]{images/ner-cout.png}
    \caption{Named entities. Left: slide 24; right: slide 26}
    \end{subfigure}\par\medskip
    \caption{Perplexity and contribution percentage of each tag by part-of-speech tags and named entity types given two consecutive checkpoints on Gutenberg PG-19 dataset. \mz{TODO: (1) simplify POS to less fine-grained categories, (2) add baselines to the contribution percentage graphs (percentage of tokens of that tag), (3) smooth the curves or use less checkpoints, (4) multiple-models or one model? (5) more datasets}}
\label{fig:pos-ner}
\end{figure}
